On the mu-invariant of anticyclotomic p-adic L-functions for CM fields

In this article, we follow Hida's approach to study the mu-invariant of the anticyclotomic projection of p-adic Hecke L-functions for CM fields along a branch character. We prove a conjecture of Gillard on the vanishing of the mu-invariant and give an exact mu-invariant formula for self-dual branch characters.

==> key_lemma.tex <==
\def\OKbasis{\bftheta}
\def\twobeta{\beta}
\def\Schar{\xi}
\section{Proof of Theorem A}\label{S:ThetaIntegral.V}
\subsection{}
In this subsection, we fix a place $v|\frakC^-$ and let $w$ be the place of $\cK$ above $v$. Let $E=\cK_v$ and $F=\cF_v$. Let $\nads_v:=\adsx_v\Abs_E^{-\onehalf}$ be a character of $E^\x$ such that $\nads_v|_{F^\x}=\tau_{E/F}$. Let $d_F$ be the generator of $\cD_\cF$ and $\delta=\delta_v=2d_F^{-1}\skewhf$ be the generator of the different $\cD_{E/F}$ fixed in \subsecref{S:different}.
\begin{lm}\label{L:key.V}Let $\beta\in F^\x$. If $A_\beta(\adsx_v)\not =0$, then
\[W(\nads_v)\tau_{E/F}(\beta)=\nads_v(2\skewhf).\]
\end{lm}
\begin{proof}
The idea is to identify $A_\beta(\adsx)$ with the Whittaker integrals of a certain Siegel-Weil section on $U(1,1)$.
Let $W=E$ with the skew-Hermitian form $\pair{x}{y}_W=\delta x\ol{y}$.
Let $G=U(W)(F)$ be the associated unitary group and let $H=U(W+W^-)(F)$, where $W^-$ is the Hermitian space $(W,-\pairing_W)$. We let $\Schar=\nads_v$ and define the induced representation $\bfI(\Schar,s)$ of $H$ by
\[\bfI(\Schar,s)=\stt{\text{smooth }f:H\to\C\mid f(\MX{a}{b}{0}{\ol{a}^{-1}}h)=\Schar(a)\abs{a}_E^{s+\onehalf}f(h)}.\]
Let $\Delta=\delta^2\in F$ and let $T=-\Delta\beta d_F^{-1}$. For $f\in\bfI(\Schar,s)$, following \cite[(6.5) p.969]{Harris:Theta_dichotomy} we define the Whittaker integral by
\[\cW_T(s)(f):=\int_F f(\MX{0}{-1}{1}{0}\MX{1}{x}{0}{1})\psi(T x)dx.\]
We embed $G$ into $H$ by
\[g\mapsto i(g,1)=\onehalf\MX{g+1}{\frac{1}{2\delta}(g-1)}{2\delta(g-1)}{g+1}.\]
Let $\Phi_{\bfone}$ be the section $\Phi_\eta$ defined in \cite[p.989 (8.6)]{Harris:Theta_dichotomy} with $\eta=\bfone$ the trivial character.
Then $\Phi_{\bfone}$ is the unique function in $\bfI(\Schar,s)$ such that $\Phi_{\bfone}(1)=1$ and $\Phi_{\bfone}(h i(g,1))=\Phi_{\bfone}(h)$ for every $g\in G$.
Recall that
\[A_\beta(\adsx_v)=\int_{F^\x}\Schar^{-1}(x+2^{-1}\delta)\abs{x+\delta}_E^{-\onehalf}\psi(-\beta d_F^{-1}x)dx.\]
By the calculation in \cite[p.990 (8.14)]{Harris:Theta_dichotomy}, we find that
\beq\label{E:3.V}\begin{aligned}\cW_T(0)(\Phi_\bfone)&=\Schar(-1)\cdot\int_F\Schar^{-1}\Abs_E^{-s-\onehalf}(x+\frac{1}{2\delta})\psi(-\Delta \beta d_F^{-1} x)dx|_{s=0}\\
&=\Schar\Abs_E^{s-\onehalf}(-2\Delta)\int_F\Schar^{-1}\Abs_E^{-s-\onehalf}(x+2^{-1}\delta)\psi(-\beta d_F^{-1}x)dx|_{s=0}\\
&=\Schar\Abs_E^{-\onehalf}(-2\Delta)\cdot A_\beta(\adsx_v).\end{aligned}
\eeq
On the other hand, let $\chi^{-c}(z):=\chi^{-1}(\zbar)$ and let $M^*(s,\Schar):\bfI(s,\Schar)\to \bfI(-s,\Schar^{-c})$ be the normalized intertwining operator defined in \cite[(6.8)]{Harris:Theta_dichotomy}. By \cite[(6.10) and Cor.\,8.3 (ii)]{Harris:Theta_dichotomy}, we have
\begin{align*}
\cW_T(0)(M^*(0,\Schar)\Phi_{\bfone})&=\tau_{E/F}(T)\cdot \cW_T(0)(\Phi_{\bfone});\\
M^*(0,\Schar)\Phi_{\bfone}&=\Schar(-\delta)\cdot W(\Schar)\cdot \Phi_{\bfone}.
\end{align*}
Therefore, it follows from \eqref{E:3.V} that \[\tau_{E/F}(-\Delta\beta d_F^{-1})\cdot A_\beta(\adsx_v)=\Schar(-\delta)W(\Schar)\cdot A_\beta(\adsx_v),\] and hence
\[ A_\beta(\adsx_v)\not =0\imply \tau_{E/F}(\beta d_F)=\Schar(-\delta)W(\Schar)\iff W(\Schar)\tau_{E/F}(\beta)=\Schar(2\skewhf).\qedhere\]
\end{proof}
\begin{prop}\label{P:6.Theta}  Suppose $v$ is inert and $w(\frakC^-)=1$. We have $v_p(A_\beta(\adsx_v))\geq \mu_p(\adsx_v)$ for all $\beta\in F^\x$. In addition, there exists $\Beth_v\in \uf^{-1}\cO_F^\x$ such that $v_p(A_{\Beth_v}(\adsx_v))=\mu_p(\adsx_v)$.
\end{prop}
\begin{proof}
Let $\stt{1,\OKbasis}=\stt{1,\bftheta_v}$ be the $\OFv$-basis of $\OKv$ fixed in \subsecref{S:different} such that $\UF=2\OKbasis$ if $v\ndivides 2$ and $\UF=\OKbasis-\ol{\OKbasis}$ if $v|2$.
Let $t=t_v=\OKbasis+\ol{\OKbasis}$ and $\addchar^\circ(x):=\addchar(-d_F^{-1}x)$. For brevity, we drop the subscript and simply write $\adsx$ for $\adsx_v$.
Since $\adsx$ is self-dual, $\adsx|_{\cO_F^\x}=1$ and $\nads(\uf)=-1$. By \cite[Prop.\,4.5 (1-3)]{Hsieh:Hecke_CM}, the formula of $A_\beta(\adsx)$ is given as follows.
\begin{mylist}
\item
If $v(\twobeta)\geq 0$ and $v(\twobeta)\not\con 0\pmod{2}$, then
\[A_\beta(\adsx)=\addchar^\circ(2^{-1}t\beta)\cdot (-1)^{v(2)+1}(1+\abs{\uf}).\]
%$A_\beta(\adsx)=c_\beta\cdot \wtd A_\beta(\adsx)$, where
%\[\wtd A_\beta(\adsx)=\begin{cases}(-1)^{v(2)+1}\addchar^\circ(t\beta)(1+\abs{\uf})&\cdots v(2)\not\con v(\beta)\pmod{2},\\
%0&\cdots v(2)\con v(\beta)\pmod{2}.
%\end{cases}\]
\item If either $v(\twobeta)<-1$ or $v(\twobeta)\con 0\pmod{2}$, then $A_\beta(\adsx)=0$.
\item If $v(\twobeta)=-1$, then
\[A_\beta(\adsx)=\addchar^\circ(2^{-1}t\beta)\cdot \abs{\uf}\sum_{x\in \bfk_F}\adsx^{-1}(x+\OKbasis)\addchar^\circ(\beta x).\]
\end{mylist}
It follows immediately that $v_p(A_\beta(\adsx))\geq v_p(1+\abs{\uf}^{-1})$ if $v(\twobeta)\not =-1$, and $v_p(A_\beta(\adsx))\geq \mu_p(\adsx)$ if $v(\twobeta)=-1$. On the other hand, note that $p$ divides $1+\abs{\uf}^{-1}$ if $\mu_p(\adsx)>0$. Thus $v_p(A_\beta(\adsx))\geq \mu_p(\adsx)$ for every $\beta\in F^\x$.

We proceed to prove the second assertion. Choose a sufficiently large finite extension $L$ of $\Qp$ so that $\adsx$ and $A_\beta(\adsx)$ for $\beta\in \uf^{-1}\cO^\x_F$ take value in $L$.
Let $e_L=v_L(p)$ and let $m=\inf_{x\in\cO_F}v_L(\adsx(x+\OKbasis)-1)=e_L^{-1}\mu_p(\adsx)$. We define the function $f:\bfk_F\to\bfk_L\subset\Fpbar$ by
\[f(\ol{x})=\uf_L^{-m}(\adsx(x+\OKbasis)-1)\pmod{(\uf_L)}.\] For $\gamma\in \cO_F$, define $\addchar_{\ol{\gamma}}:\bfk_F\to \Fpbar$ by $\addchar_{\ol{\gamma}}(x)=\addchar^\circ(\frac{\gamma}{\uf}x)\pmod{\frakm}$.
Then $\stt{\addchar_{\ol{\gamma}}}_{\ol{\gamma}\in \bfk_F}$ gives a $\Fpbar$-basis of the space of $\Fpbar$-valued functions on $\bfk_F$. Then $f$ can be uniquely written as
$f(x)=\sum_{\ol{\gamma}\in\bfk_F}c_\gamma(f)\addchar_{\ol{\gamma}}(x)$, where $c_\gamma(f)$ is the $\ol{\gamma}$-coefficient of $f$ given by
\begin{align*}c_\gamma(f)&=\abs{\uf}\sum_{x\in\bfk_F}f(x)\psi_{\ol{\gamma}}(x)=\uf_L^{-m}\abs{\uf}\sum_{x\in\bfk_F}\adsx^{-1}(x+\OKbasis)\psi^\circ(\frac{\gamma}{\uf}x)\\
&=\uf_L^{-m}\addchar^\circ(-2^{-1}t\beta)\cdot A_{\gamma\uf^{-1}}(\adsx)\pmod{\frakm_L}.\end{align*}
Since $f$ is a non-zero function by definition, some $\ol{\gamma}$-coefficient of $f$ is nonzero, namely  $c_{\gamma}(f)\not\con 0\pmod{\frakm_L}$.
Let $\Beth:=\gamma \uf^{-1}$. Then $v_L(A_{\Beth}(\adsx))=m$ and hence $v_p(A_{\Beth}(\adsx))=\mu_p(\adsx)$.
\end{proof}

The following proposition is the key ingredient in our proof.
\begin{prop}\label{P:NVAbeta.V}%For every $v|\frakC^-$,
There exists $\Beth_v\in F^\x$ such that
\begin{itemize}
\item[(i)] $v_p(A_{\Beth_v}(\adsx_v))=\mu_p(\adsx_v)$,
\item[(ii)] $W(\nads_v)\tau_{E/F}(\Beth_v)=\nads_v(2\skewhf)$.
%\item  \[v(\beta)=-v(d_F)-2+\begin{cases}k&\cdots \text{ $E/F$ is ramified},\\
%2k&\cdots \text{ $E/F$ is unramified and $n(\psi')$ is even},\\
%2k-1&\cdots\text{ $n(\psi')$ is odd}.\end{cases}\]
\end{itemize}
\end{prop}
\begin{proof}
When $w(\frakC^-)=1$ and $v$ is inert, (i) is verified in \propref{P:6.Theta}. Suppose that either $w(\frakC^-)>1$ or $v$ is ramified. Then we must have $\mu_p(\adsx_v)=0$ as $v\ndivides p$ and $p>2$. By \cite[Lemma 6.4]{Hsieh:Hecke_CM}, there exists $\Beth_v\in F^\x$ such that $A_{\Beth_v}(\adsx_v)\not\con 0\pmod{\frakm}$. Thus $v_p(A_{\Beth_v}(\adsx_v))=\mu_p(\adsx_v)=0$. To show the epsilon dichotomy property (ii) for this $\Beth_v$, we
note that (i) implies that $A_{\Beth_v}(\adsx_v)\not =0$ ($\adsx_v$ is ramified), and (ii) follows from \lmref{L:key.V}.
\end{proof}
\begin{Remark}In virtue of \cite[Prop.\,6.7]{Hsieh:Hecke_CM}, \propref{P:NVAbeta.V} removes the assumption (C) in \cite[Thm.\,6.8]{Hsieh:Hecke_CM}.
\end{Remark}
\subsection{}
Now we are ready to prove our main theorem.
\begin{thm}\label{T:main.V}Suppose that $p\ndivide D_{\cF}$. Let $\adsx$ be a self-dual Hecke character of $\cK^\x$ such that \HypMu
Then
\[\Imu^-=\sum_{v|\frakC^-}\mu_p(\adsx_v).\]
%If we suppose further that $p\ndivides h_\cK^-$, then the equality holds.
\end{thm}
\begin{proof}
In view of \eqref{E:FA.V} and \propref{P:6.Theta}, we find that \[v_p(\bfa_\beta^\setp(\adsx,\frakc(a)))\geq \sum\limits_{v|\frakC^-}\mu_p(\adsx_v)\text{ for all }\beta\in\cF_+\text{ and }a\in\cD_1.\]
Combined with the formula \eqref{E:fourierformula.E} of $\bfa_\beta(\Eadsu,\frakc(a))$ and \thmref{T:1.V}, this implies that
\beq\label{E:10.V}\Imu^-\geq \sum_{v|\frakC^-}\mu_p(\adsx_v).\eeq

For each $v|\frakC^-$, we let $\Beth_v$ be as in \propref{P:NVAbeta.V}. Then
$v_p(A_{\Beth_v}(\adsx_v))=\mu_p(\adsx_v)$ and $W(\nads_v)\qchKF(\Beth_v)=\nads_v(2\skewhf)$ for every $v|\frakC^-$.
From the assumption that $W(\nads)=\prod_v W(\nads_v)=1$ we can deduce that there exists $\beta\in\cF_+$ such that
\begin{enumerate}
\item $\beta\in\cO_{\cF,(p\Csplit\Csplit^c)}^\x$,
\item $A_\beta(\adsx_v)=A_{\Beth_v}(\adsx_v)$ for every $v|\frakC^-$,
\item $\prod_{\frakq|\frakC^-}\frakq^{v_\frakq(\beta)}=(\beta)\frakc(\OK)\rmN_{\cK/\cF}(\fraka)$ for some prime-to-$p\frakC$ ideal $\fraka$ of $\OK$.
\end{enumerate}
(\cf \cite[Prop.\,6.7]{Hsieh:Hecke_CM}.) Let $\bfc\in\AFf^\x$ be the idele such that $\bfc_v=\beta^{-1}$ for all $v\ndivide p\frakC\frakC^c$ and $\bfc_v=1$ if $v|p\frakC\frakC^c$. Then $\frakc(\fraka):=\il_\cF(\bfc)=\frakc(\OK)\rmN_{\cK/\cF}(\fraka)$ is the ideal corresponding to $\bfc$. Let $u\in\cU_p$ such that $u\con\beta\pmod{p}$. By \eqref{E:FA.V} and \eqref{E:fourierformula.E}, we find that
\beq\label{E:11.V}v_p(\bfa_\beta(\Eadsu,\frakc(\fraka)))=\sum_{v|\frakC^-}v_p(A_\beta(\adsx_v))=\sum_{v|\frakC^-}v_p(A_{\Beth_v}(\adsx_v))=\sum_{v|\frakC^-}\mu_p(\adsx_v).\eeq
Combining \thmref{T:1.V}, \eqref{E:10.V} with \eqref{E:11.V}, we obtain
\[\Imu^-=\sum_{v|\frakC^-}\mu_p(\adsx_v).\qedhere\]
\end{proof}


